LLMShot: Reducing snapshot testing maintenance via LLMs

Snapshot testing has emerged as a critical technique for UI validation in modern software development, yet it suffers from substantial maintenance overhead due to frequent UI changes causing test failures that require manual inspection to distinguish between genuine regressions and intentional design changes. This manual triage process becomes increasingly burdensome as applications evolve, creating a need for automated analysis solutions. This paper introduces LLMShot, a novel framework that leverages Vision-Language Models (VLMs) to automatically analyze snapshot test failures through semantic classification of UI changes. To evaluate LLMShot's effectiveness, we developed a comprehensive dataset using a feature-rich iOS application with configurable feature flags, creating realistic scenarios that produce authentic snapshot differences representative of real development workflows. Our evaluation using Gemma3 models demonstrates strong classification performance, with the 12B variant achieving over 84% recall in identifying failure root causes while the 4B model offers practical deployment advantages with acceptable performance for continuous integration environments. However, our exploration of selective ignore mechanisms revealed significant limitations in current prompting-based approaches for controllable visual reasoning. LLMShot represents the first automated approach to semantic snapshot test analysis, offering developers structured insights that can substantially reduce manual triage effort and advance toward more intelligent UI testing paradigms.

==> analysis_ex.tex <==
\begin{lstlisting}[caption={Analysis output for EnhancedSettings test},label={lst:analysis_ex}]
"EnhancedSettings": {
    "reasons": [
      "LAYOUT_CHANGE",
      "COLOR_CHANGE",
      "UNKNOWN-UI_elements_misalignment"
    ],
    "pixel_diff": 0.85,
    "semantic_diff": 0.75,
    "affected_elements": [
      "Enable Notifications toggle",
      "Dark Mode switch",
      "Account Type label"
    ],
    "explanation": "The primary cause of the failure is a layout change, specifically a misalignment of UI elements. The ‘Enable Notifications’ toggle and the ‘Dark Mode’ switch are noticeably misaligned in the failure image compared to the reference. The ‘Account Type’ label also exhibits a slight misalignment. While pixel-wise differences are significant (85%), a substantial portion of the UI components appear to be functionally the same, suggesting a fundamental layout issue. The pixel differences primarily reflect the misalignment, rather than a change in color, font, or other semantic changes.",
    "_metadata": {
      "test_directory": "EnhancedSettings",
      "timestamp": "2025-05-04T10:08:15.175845",
      "model": "gemma3:4b",
      "model_version": "unknown",
      "possible_categories": [
        "LAYOUT_CHANGE",
        "COLOR_CHANGE"
      ],
      "run_id": "gemma3_4b_2025-05-04T10:08:15.175845",
      "ground_truth": {
        "pixel_difference": 0.12542241295670514
      },
      "performance": {
        "response_time_seconds": 9.243278,
        "confidence_score": 0.5,
        "has_unknown_categories": true,
        "pixel_diff_accuracy": 0.2754224129567051
      }
    }
}
\end{lstlisting}

==> feat_flag_lst.tex <==
\begin{lstlisting}[caption={An example feature flag implementation, showcasing how we dynamically change our code during tests},label=lst:featureflag]
Text(
  (FeatureFlags.isEnabled(.CONTENT_CHANGE_WELCOME_MESSAGE)
      ? "Welcome back, \(stateManager.userType == .premium ? "Premium User" : "User")!"
      : stateManager.greeting)
)
\end{lstlisting}

==> fig_snapshots.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{ex-snapshots.png}
    \caption{An example reference, failure and diff image for a \texttt{COLOR\_CHANGE}. The blue toggle color is now red in the failure snapshot.}
    \label{fig:snapshots}
\end{figure}

==> intro_comments.tex <==
%Snapshot testing is a new form of testing that has gained popularity in recent years (Panchuk, 2022). Essentially, it can be used as a User Interface (UI) test that compares the current state of the interface to a previously stored state (or snapshot). By adopting snapshots tests, developers aim to detect unexpected UI changes without devoting a major effort designing and implementing tests with complex and detailed assertions. 
%Snapshot tests are an emerging software testing approach that rapidly became widely adopted by many and important software organizations. The significance of snapshot testing in practice can be illustrated by the number and importance of the software companies that are using this type of test. For example, Airbnb’s iOS app has approximately 30,000 snapshot tests, which is three times greater than the number of unit tests in the app. As other examples, Spotify and Shopify apps have more than 1000 snapshot tests Additional examples of companies using snapshot tests include Uber, Lyft, and Robinhood.

%Snapshot tests are mostly adopted due to their easiness of implementation, which allows developers to write more tests and consequently prevent regressions in their projects. 2. The most common drawback is the fragility of snapshot tests, leading to the necessity of constant updates of the ‘‘golden standard’’ snapshot.
%According to our findings, snapshot tests are easy to implement and at the same time, they can be effective to prevent regressions. They are also serializable, which makes their result comprehensible and subject to code reviews. For this reason, they are seen as an alternative to UI tests implemented using tools such as Cypress and Playwright. However, the simplicity and easiness of implementation come at the price of being fragile and therefore subjected to false positives. \cite{snapshot_lit}


%In modern software development, snapshot testing has become a popular approach, especially in environments where program changes occur often [50]. Software development teams face great difficulty in handling rapid code changes while making sure that these changes also don’t inadvertently bring unexpected problems or regressions into the codebase they work in due to the growing need for more dynamic applications [30]. Snapshot testing addresses this challenge by capturing the state of an application component at a particular instant in time and comparing it with a previously recorded snapshot. This comparison allows developers to swiftly identify possible differences in the output of a component, which provides an effective method for detecting potential defects that were not intended in the first place, providing an efficient way to detect unintended regressions [16, 7].1

%Snapshot testing has been adopted by large scale applications developed by industry leaders such as Airbnb2, Spotify3, and Shopify4, with the intention of maintaining a high level of quality for features that are perceived by users It has been reported, for instance, that the native iOS app of Airbnb contains as many as tens of thousands of snapshot tests. here are a few specific pieces in academic literature that have been written specifically for snapshot testing. In contrast, there is substantial grey literature on this topic written by industry practitioners and software developers\cite{snapshot_lit}

%When it comes to software testing, snapshot testing is used particularly for user interface components, where it is considered essential to preserve both visual and behavioral consistency for user-facing feature. One of the most important aspects of snapshot testing is the process of taking a snapshot of the output of a component. For this reason, snapshot testing is considered a type of golden master testing. After taking a first snapshot, every time the test runs it compares the current state of the component under test to the stored snapshot. If the two instances remain identical, the test passes. Otherwise, it fails

%Testing frameworks such as Jest have the option of encoding snapshots into a file, making it simpler to check the tests on further runs, and also working as an artifact to be reviewed as part of a code review process

%The roots of snapshot testing can be traced back to broader testing practices outlined in Feathers’ work on software maintenance, particularly in his discussion of characterization testing [19]. Feathers introduces characterization testing as a strategy for understanding and preserving existing system behavior when making code modifications, especially in legacy systems. This approach emphasizes creating tests that characterize the current behavior of a system, allowing developers to detect unintended changes without needing complete knowledge of the underlying code [19]. Snapshot testing builds on this principle by capturing a snapshot of a component’s output, aligning with the goals of characterization testing, and helping developers confidently refactor or enhance code by providing a reliable mechanism to catch regressions. Snapshot testing may not be just a tool for detecting regressions but part of a broader framework that helps safeguard and understand system behavior during development.


%we discovered that snapshot testing has many benefits, as it is considered easy to implement and has the ability to prevent regressions effectively, by constantly detecting changes. Also, this testing technique provides a fair amount of flexibility for its snapshots when comparing different data types like DOM trees, serialized images, or JSON blobs. This versatility allows developers to capture the exact output of complex data structures and user interfaces, ensuring consistency over time.

%evealed significant drawbacks, the most notable being the fragility of snapshot tests. This fragility derives from a dependency on the exact component output, leading to frequent false positives as minor updates often cause test failures. Developers must carefully evaluate differences to determine if they represent genuine issues or otherwise expected changes, a challenge that can lower confidence in the test suite. Additionally, large snapshots and lack of context further complicate debugging, particularly for developers unfamiliar with the tested component.

%napshot testing serves an interesting purpose in the software testing field, valued for its ease of use and effectiveness in preventing regressions, especially in frontend development. Nonetheless, the quick setup and simplicity of this technique may result in much reliance, possibly obscuring underlying problems when snapshots are updated too aggressively. Consequently, developers encounter the challenge of reconciling the ease of snapshot testing with the necessary care to uphold its integrity over time.

%Changes to code often lead to failing tests, as the snapshots may need frequent updates to align with intended modifications. This fragility can result in a high incidence of false positives, prompting developers to blindly update snapshots without thoroughly verifying the nature of each change. Additionally, snapshots can become challenging to manage when they grow large, complicating code reviews and possible merge conflict resolutions. The lack of context in snapshot tests, often caused by minimal or unclear descriptions when written, further complicates debugging when test failures occur.

%These findings highlight the importance of maintaining a clear and manageable structure in snapshot tests by breaking large snapshots into smaller ones with more detailed descriptions, yet their effectiveness still largely depends on the care with which tests are written and maintained by software developers. This highlights the necessity for more comprehensive and strict guidelines while crafting snapshot tests that remain robust over time, ensuring they continue to serve their original purpose without slowly becoming a maintenance burden.

%uch as ease of implementation, regression detection, and improved test automation Similarly, the drawbacks reported in RQ3.2—such as test fragility, excessive main- tenance overhead, and lack of meaningful assertions
%---

%In recent years, snapshot testing, which compares snapshots of UI components to detect unexpected changes, has gained popularity in front-end development due to the need to reduce testing efforts.

%More recently, snapshot testing has gained popularity in front-end development due to the need of reducing testing effort. Specifically, major companies including Amazon, Google, and Microsoft have adopted snapshot testing [1].

%Snapshot testing is a type of output comparison testing technique that asserts whether the outputs by the current state of the product remain unchanged. That is, it only detects differences before and after code changes, and ignores whether the current state is correct. The aim of snapshot tests differs from those of unit and functional tests that define the correct behavior of the products.

%Snapshot tests require little time to create because developers can just take snapshots of UI components when the current version of the product is considered ideal [2]. The ideal state will be compared with the future state of UI components. Given the ability of detecting unexpected changes in UI, it can be applied in different scenarios. For example, React components are often shared by multiple UIs, applying snapshot testing can help ensure no dependents will break.

%While snapshot testing is widely adopted in practice and the community is still growing rapidly, researchers have paid little attention to it.

%This study presents an empirical investigation on the use of snapshot tests xamine the characteristics of projects using snapshot tests, as well as the adoption and evolution of snapshot tests.\cite{emp_study_snapshot}

%While various types of tests including unit tests, integration tests, and GUI tests have been studied by researchers [3] [4] [5] [10], only a few of them [2] [11] have focused on snapshot testing.

%Bui and Rocha [11] published a dataset of repositories using JEST’s snapshot files. They identified JEST adoption by checking whether the GitHub repository uses the tag of “jest”. Their data includes attributes from the latest commit of projects (e.g., the number of stars, issues, snap files, test files). Cruz et al. [2] conducted a grey literature review in order to investigate the adoption of snapshot testing in practice, revealing trade-offs and best practices. They found that snapshots are simple to create and can prevent regressions while they may easily become fragile if used improperly.

%---
%Snapshot testing is a form of software testing that is focused on visual components by highlighting any code changes when compared to a previously stored state This quick and simple method of testing is growing popular among the industry with companies such as Spotify and Robinhood. Despite its growing popularity, snapshot testing is barely explored in academia

%Snapshot testing focuses on testing the visual components of a software. It involves taking a “snapshot” or stored state and comparing it to the current visual code output. This method helps developers notice any changes in the interface components of their code, whether it is intentional or not. If it is intentional, they can quickly update the stored state, otherwise, the snapshot test highlights the differences in the code elements

%Snapshot testing is growing popular in industry with major companies like Spotify with around 1,600 snapshot tests, Robinhood with around 400 snapshot tests, and Shopify with around 2,300 snapshot tests [7]. The tests are shorter, easier to maintain and easy to use. To update a snapshot, it only takes one singular command

%To check to make sure components of a program do not change unexpectedly, developers would need to create tests to cover every and all scenarios in a program [9]. In order to minimize the amount of time needed to perform these tests, many developers have adopted the practice of Snapshot Testing with the rise of testing frameworks capable of performing this activity. Snapshot Testing, traditionally referred to as visual regression testing, compares the current values of visual components to previously stored ones, and is commonly used and supported by tools such as Jest and Cypress


%By taking a snapshot of the visual component code output, the program is then able to compare it to following captures. The test fails if the two snapshots have any perceivable differences, and succeeds if they do not. If it fails, the program will indicate where lies the difference between the two. These changes can either be deliberate, in which then the stored snapshot should be updated, or unintentional, in which the test discovered an inconsistency in the code

%Snapshot testing is not only easy, but also fast to write, making it a desirable testing strategy for developers. Writing tests in this manner tends to be faster than traditional unit tests, and easier to use [5], since developers only need to check flags to see whether a snapshot is the same as the stored version [9]. Additionally, the snapshots are easy to update with a single command, rather than needing to edit multiple files

%This form of testing however, comes with its drawbacks. Any changes, even if they are insignificant, will cause snapshot tests to fail and will require developers to manually verify that everything is working properly. Because these tests only take into account changes, it does not indicate whether the output is "correct", and therefore, cannot be a complete substitute for unit testing. These snapshots also must be stored somewhere, but fortunately, they typically do not take up too much space

%Snapshot testing is a very new topic in academia, and consequently, there are few academic references for it.Figueiredo et al. [12] creates an approach to validate Android software builds. The authors use the screenshots of the built software into machine learning techniques to identify potential problems and whether the built was valid. The authors briefly mention snapshot testing in their background Although the authors’ approach is a form of visual regression testing, it differs from snapshot testing which detects dissimilarities in the programming code of visual elements instead of using screenshots.

%---
%https://www.sitepen.com/blog/snapshot-testing-benefits-and-drawbacks Snapshot tests are fundamentally different from unit and functional tests. While these types of tests make assertions about the correct behavior of an application, snapshot tests only assert that the output now is the same as the output before; it says nothing about whether the behavior was correct in either case.

%The term has traditionally referred to visual regression testing, where a literal snapshot of a rendered app or page is compared to a stored image. However, Jest’s render tests are what really brought the term into the mainstream for modern front-end developers, and this is what “snapshot testing” typically means in the JavaScript world.

%While snapshot tests are easier to write and keep up to date than traditional unit or functional tests, and they can be an effective tool for preventing regressions in an application, they do have several potential drawbacks.

%A significant disadvantage is that they’re tightly coupled to an application’s output, making them very fragile. Any changes, even to insignificant parts of the output, can cause snapshot tests to fail. Developers then must (or at least should) manually verify that everything is still working properly and update the snapshots.

%This leads to another potential problem with snapshot tests: they don’t actually indicate anything about the expected output, just that it shouldn’t change. Unlike unit and functional tests, snapshot tests don’t contain focused, meaningful assertions or expectations. A developer who has to manually verify that the output is still “good” may run into trouble when the failing test is for a part of the app he or she isn’t familiar with, because a snapshot test doesn’t indicate what parts of the output are important.

%Snapshot tests aren’t inherently well suited to dynamic content. A “random quote of the day” component will frequently fail snapshot tests since the random quote in the output usually won’t match the stored component data. Tools can deal with this problem by letting users mark areas with dynamic content.

%---
%https://jestjs.io/docs/snapshot-testing
%Snapshot tests are a very useful tool whenever you want to make sure your UI does not change unexpectedly.

%A typical snapshot test case renders a UI component, takes a snapshot, then compares it to a reference snapshot file stored alongside the test. The test will fail if the two snapshots do not match: either the change is unexpected, or the reference snapshot needs to be updated to the new version of the UI component.


%---
%https://jestjs.io/blog/2016/07/27/jest-14
%we use a system called “snapshot testing”: a snapshot test system that renders UI components, takes a screenshot and subsequently compares a recorded screenshot with changes made by an engineer. If the screenshots don't match, there are two possibilities: either the change is unexpected or the screenshot can be updated to the new version of the UI component.

%---
%https://benmccormick.org/2016/09/19/074100.html
%UI components often change in small and trivial ways. Copy is changed, whitespace is added, a border color is modified. Generally this means that developers have to choose between detailed tests that catch any regression but require constant updates, or less detailed tests that focus on core behaviors but miss smaller regressions.

%Snapshot tests provide a new way of approaching these problems in unit tests. Because they are easy to write and effortless to update, and provide a clear view of what changed after each update, whether it is major or minor.
%---
%https://jestjs.io/blog/2016/07/27/jest-14
% a snapshot test system that renders UI components, takes a screenshot and subsequently compares a recorded screenshot with changes made by an engineer. If the screenshots don't match, there are two possibilities: either the change is unexpected or the screenshot can be updated to the new version of the UI component.

% ---
% Snapshot tests compare a screen’s layout or a UI element with a reference image of the expected result. They’re a valuable, and increasingly popular, middle ground between unit and UI tests. They’re easy to write, run faster than UI tests, and are very visual to debug, since you just need to compare two images. These tests can help catch visual regressions in the development life cycle, which isn’t possible with unit or UI tests. 


%Apps are getting increasingly more complex. To make code changes under this complexity, programmers have been writing tests for a good while now. Recently, Snapshot Testing (ST) was proposed as an alternative to UI-presence tests. In UI tests, each coding framework provides their own action-simulation API for their GUI elements, and the programmers can simulate actions like tapping, right click or swipes etc. A presence test checks whether a UI element in view is present, or satisfies a given condition. While this approach is a straightforward way to automatically validate some state and navigation changes, it falls short in many areas. First, such tests are generally very tedious to write, since every single element of importance must be manually coded to be checked. Second, we can only check very general facts about a view's state. In cases where the state or the look of the view is complex and dynamic, there are no obvious ways to validate their state. In comparison, snapshot tests take a snapshot of the view state at a predetermined program state, and the subsequent tests check the similarity with this baseline (See Figure \ref{fig:snapshot_flow}). While a snapshot can also mean the textual representation of the view hierarchy, this study strictly deals with snapshots that are screenshots of the view under test. Using this snapshots, UI tests are enabled to detect even small padding or color changes in the UI without writing any view-specific code.


%While snapshot tests provide a very simple, fast and explainable way of writing UI tests, they also have their downsides. Since snapshot tests work by comparing the freshly taken snapshot to a baseline reference snapshot, any change to the UI, whetter it is due to an intentional or unintentional change, will cause a snapshot missmatch. In such cases, the feature implementer should also change the reference snapshot along with the intended code change, after manually making sure that the newly created baseline snapshot looks as intended. The code reviewers should also be vigilant of any unintended change to the these baseline snapshots. Although all test code is bound to change with the change in software requirements, changing snapshot test baselines could be more open to human errors, and might be slower. This recreation process also takes significant time, with around 8.2\% of the commits are just made for regenerating reference snapshots \cite{emp_study_snapshot}.
%\ak{what is the gap we are tryin to adress, what is the problem statement, why this study is necessary?}
%\ak{introduce our approach.}
%LLMShot is a powerful tool designed to change the approach to UI testing and validation, and alleviate the shortcomings of the traditional approach. By leveraging LLMs to analyze visual differences between baseline and current snapshots, this framework provides insights into UI regressions to help developers understand why a snapshot similarity check failed, and also direct the focus of the similarity change based on natural language directives. Unlike traditional snapshot testing tools that simply flag binary pass/fail results, LLMShot employs Gemma3 to categorize, quantify, and explain visual discrepancies and assigns a smart pass/fail label based on developer preferences. \\

%Research Gap and Motivation
%Despite the widespread adoption of snapshot testing in modern software development, particularly for user interfaces, the current practice suffers from several key limitations. Traditional snapshot tests are binary in nature—they indicate only whether a change has occurred, without providing context or explanation. This often leads to false positives, as even trivial, non-functional differences trigger test failures. Developers must then manually inspect differences, determine whether the changes are significant, and decide whether to update the snapshot. This process is time-consuming, error-prone, and increasingly unmanageable as applications and test suites grow in size.

%Moreover, the lack of semantic insight in existing tools means they cannot distinguish between meaningful visual regressions and inconsequential changes, nor can they adapt to specific developer expectations or evolving UI designs. This fragility and lack of interpretability create a maintenance burden, and undermine confidence in the value of snapshot testing.

%Problem Statement
%While snapshot testing remains a popular tool for regression detection in UI development, its effectiveness is limited by its inability to explain why a test failed or what the failure actually means. The binary nature of the results, combined with the absence of contextual understanding, makes it difficult for developers to efficiently triage and address failures. This lack of semantic interpretation and configurability represents a significant barrier to the broader utility and reliability of snapshot testing in modern development pipelines.

%Our Approach: LLMShot
%To address these shortcomings, we propose LLMShot, a novel framework that augments traditional snapshot testing with the interpretive capabilities of large language models (LLMs). LLMShot integrates Gemma-3, a state-of-the-art vision-language model, to perform semantic analysis of visual differences between baseline and current snapshots. Instead of offering a simple pass/fail outcome, LLMShot:

%Categorizes and quantifies visual discrepancies,

%Provides natural language explanations for detected changes,

%Supports developer-defined preferences for what constitutes an acceptable change, and

%Assigns smart pass/fail labels that reflect these preferences rather than arbitrary pixel differences.

%By interpreting snapshot differences through the lens of natural language and contextual reasoning, LLMShot offers a more robust, interpretable, and customizable testing experience. It not only helps developers understand the nature and relevance of changes, but also reduces noise in test results, lowers maintenance overhead, and improves confidence in the UI validation process.

% Using LLMShot, this research focuses on the following research questions:
% \begin{description}
%   \item[RQ1] Can visual‑LLMs automatically classify the root cause of snapshot test failures and provide actionable explanations?
%   \item[RQ2] Does the \textit{ignore‑category} mechanism meaningfully reduce false‑positive snapshot failures while preserving fault detection?
%   \item[RQ3] What is the trade‑off between model size (4B vs.\ 12B parameters) and analysis accuracy/latency when integrating visual‑LLMs into CI pipelines?
% \end{description}



%We build a SwiftUI demo app and run 17 UI tests across multiple feature‑flag permutations, producing paired \textit{reference}, \textit{failure}, and \textit{diff} screenshots plus rich metadata.  
%These triplets are processed by a Python pipeline that queries Gemma3‑based vision‑LLMs, which return structured JSON containing change categories, pixel/semantic scores, affected elements, and explanations.

%LLMShot reliably categorises snapshot mismatches, supplies developer‑friendly explanations for the detected defects, and via the ignore mechanism, reduces baseline updates by suppressing expected changes. The 4B model achieves comparable accuracy to the 12B variant in defect categorization (\% Accuracy), while analysing a snapshot triplet in a few seconds on a laptop‑class GPU, making local CI integration practical.


%Despite the popularity of snapshot testing, the current state of the art lacks a nuanced approach to understanding visual discrepancies. Developers are often left with binary pass/fail results that do not explain the nature of changes between snapshots, leading to:

%Frequent false positives: Minor UI adjustments can cause snapshot tests to fail, requiring unnecessary snapshot updates without verifying whether the change was intentional.

%Difficulty in pinpointing causes: When discrepancies occur, it is hard to identify which specific components have been affected or whether the change is expected.

%Inefficient integration with dynamic UI components: As modern applications feature dynamic and complex UIs, traditional snapshot testing frameworks struggle to adapt, creating a maintenance burden.

%Thus, a more intelligent, contextual approach to snapshot testing is needed—one that not only identifies changes but also explains their causes, simulates different UI states, and allows for a smarter and more efficient testing workflow.

%LLMShot aims to overcome the shortcomings of traditional snapshot testing by incorporating advanced large language models (LLMs) into the analysis of visual discrepancies. Unlike traditional snapshot testing tools, which only flag mismatches between snapshots, LLMShot:

%Classifies and explains snapshot mismatches: It categorizes the cause of the discrepancy, providing detailed explanations and a list of the affected UI components.

%Simulates defect absence: It allows for the simulation of missing UI defects, helping developers to reevaluate test results based on the semantic difference between the original and simulated snapshots.

%Adapts to real-world scenarios: Despite relying on models with as few as 4 billion parameters, LLMShot demonstrates fast and efficient performance, making it suitable for local, real-time evaluation in development environments.

%This approach enhances the developer’s understanding of UI regressions, allowing them to focus on contextual differences rather than simply flagging binary failures. Additionally, by leveraging natural language processing, LLMShot provides developers with actionable insights into the changes and their significance.

%Our contributions in this study are as follows:

%LLM-based Intelligent Snapshot Analysis System: We introduce a novel system that leverages large language models (LLMs) to enhance traditional snapshot testing:

%Accurate mismatch classification: The system accurately classifies the cause of snapshot mismatches, provides detailed explanations, and lists affected UI components.

%Defect absence simulation: It simulates the absence of certain UI defects, allowing the test result to be reevaluated based on the semantic differences between the current and simulated states.

%Efficient performance: The framework performs well even with 4-billion-parameter models, ensuring local, fast evaluation.

%Feature-Rich iOS Demo App:
%We provide a comprehensive iOS demo application showcasing real-world features that challenge traditional snapshot testing, helping to demonstrate the applicability of our approach in complex scenarios.

%Robust and Easy-to-Use Command-Line Interface (CLI):
%We present a user-friendly CLI that facilitates easy integration of our intelligent snapshot analysis system into existing testing workflows, making it simple to adopt our approach in real-world development environments.

%5. Conclusion
%Snapshot testing has proven to be a valuable technique for detecting regressions in UI components. However, the traditional approach has limitations, especially in handling the growing complexity of modern applications. By integrating large language models, LLMShot addresses these limitations, offering more intelligent, actionable insights into snapshot mismatches. Through accurate classification, defect simulation, and fast performance, LLMShot not only improves the testing process but also reduces the overhead associated with managing UI regressions.

%Our approach opens the door to more efficient and reliable snapshot testing, and we hope that our contributions will inspire future research and development in this area, ultimately enhancing the software testing landscape for dynamic, modern applications.

%The rest of this article is structured as follows: In Section II, we review GUI testing and visual‑oracle literature. Section III presents the LLMShot methodology, dataset, and analysis pipeline. Section IV details the experimental setup empirical evaluation, while Section V discusses these findings and limitations. We present our threats to validity in Section VI, and conclude the article with Section VII with a brief discussion on future work direction.

%Despite the popularity of snapshot testing, the current state of the art lacks a nuanced approach to understanding visual discrepancies. Developers are often faced with:

%Mismatch identification without context: Traditional snapshot tests identify changes but don’t provide detailed insights into why those changes occurred or which specific UI components were affected.

%Frequent false positives: Minor, insignificant UI adjustments can cause snapshot tests to show differences, leading developers to frequently update snapshots without verifying whether the changes were intentional.

%Difficulty in pinpointing causes: While snapshot tests show diffs between the current and baseline snapshots, they don’t explain the underlying reasons for the mismatch, making it harder to assess whether the change is a regression or an expected modification.

%Inefficient handling of dynamic UI components: As modern applications feature increasingly dynamic and complex UIs, traditional snapshot testing tools struggle to effectively address these challenges, often resulting in higher maintenance overhead.

%Thus, a more intelligent, contextual approach to snapshot testing is needed—one that not only identifies visual differences but also provides insight into their causes, reduces false positives, and supports dynamic UI changes efficiently.
%---

%Snapshot testing has become a widely adopted technique in modern software development, particularly for validating user interfaces (UIs). By capturing and comparing screenshots of UI components at different stages of development, snapshot testing can automatically detect regressions and discrepancies, ensuring that the UI remains consistent. However, despite its popularity, current snapshot testing practices face significant limitations that hinder their effectiveness and scalability in real-world applications.

%Problem Statement
%Traditional snapshot tests focus solely on identifying visual differences between baseline and current snapshots. While this provides a basic mechanism for regression detection, it lacks contextual information, making it difficult for developers to interpret the results meaningfully. Specifically, traditional snapshot tests:

%Do not provide detailed explanations: A failure simply indicates a difference, but it doesn’t explain the cause of the difference, whether it's a significant regression, an intentional update, or an inconsequential UI tweak.

%Suffer from frequent false positives: Minor, non-functional changes (such as styling adjustments or layout shifts) can trigger failures, leading developers to update snapshots without verifying whether the change was intentional or impactful.

%Lack adaptability: As UIs become more dynamic and complex, the static nature of snapshot testing struggles to handle changes in state, content, or interaction, resulting in an ever-increasing maintenance burden.

%These issues have created a gap in the ability of snapshot testing to scale with the growing complexity of modern applications. The lack of semantic understanding in existing tools limits the efficiency and reliability of snapshot testing, especially in large-scale, fast-evolving projects.

%Related Work and Literature Gap
%Snapshot testing has a rich history, with tools like Jest and Percy providing essential regression detection capabilities. However, most existing approaches rely on pixel-perfect comparisons, which are inherently brittle. They cannot distinguish between meaningful changes (e.g., functional updates) and trivial differences (e.g., text alignment or background color changes). Other efforts have sought to improve snapshot testing by introducing visual or semantic analysis, but these approaches often lack integration with the broader developer workflow or fail to provide actionable insights. Furthermore, many existing tools struggle to accommodate the complexity of modern, dynamic UIs, which feature components that change based on user interaction, device orientation, or feature flags.

%This leaves a significant gap: While snapshot testing is valuable for regression detection, current practices offer limited interpretability, configurability, and adaptability, making them less effective in real-world, large-scale projects.

%Our Novelty
%In this paper, we propose LLMShot, a novel framework that augments traditional snapshot testing with the semantic and interpretive power of large language models (LLMs). LLMShot combines the capabilities of state-of-the-art vision-language models, such as Gemma-3, to analyze and explain visual discrepancies between baseline and current snapshots. Rather than simply flagging changes, LLMShot offers several key improvements over traditional snapshot testing:

%Semantic Analysis: LLMShot categorizes visual discrepancies and provides natural language explanations for detected changes, helping developers understand not just that a change has occurred, but why and what was affected.

%Contextual Adaptability: The framework allows developers to define what constitutes an acceptable change, providing flexibility to handle dynamic UI states and ongoing design evolutions.

%Efficient Performance: By leveraging compact LLMs (as small as 4 billion parameters), LLMShot maintains fast performance and low latency, making it suitable for real-time integration into development pipelines.

%LLMShot is designed to make snapshot testing smarter, more interpretable, and more scalable. By providing contextual, semantic insights into visual changes, LLMShot reduces noise in test results, enhances the developer experience, and ultimately leads to more efficient UI validation.

%Contributions
%This paper makes the following contributions:

%LLM-based Intelligent Snapshot Analysis:

%Accurate Mismatch Classification: LLMShot uses LLMs to classify the root causes of snapshot mismatches, providing detailed explanations and highlighting affected UI components.

%Defect Absence Simulation: LLMShot can simulate the absence of certain UI defects, allowing for a more nuanced reevaluation of test results based on the semantic difference between the current and simulated states.

%Scalable and Efficient: LLMShot performs effectively with models as small as 4 billion parameters, ensuring that developers can integrate it into their workflows without sacrificing speed or accuracy.

%Real-World iOS Demo App:

%We present an iOS demo app that illustrates real-world features and UI complexities that challenge traditional snapshot tests. This app serves as a testing ground for LLMShot, showcasing its practical application in complex, dynamic environments.

%Easy-to-Use Command-Line Interface (CLI):

%To simplify integration, we provide a robust CLI that enables seamless adoption of LLMShot into existing testing frameworks, ensuring that developers can quickly incorporate the system into their CI/CD pipelines.

%---

==> metadata.tex <==
\begin{lstlisting}[language=JSON, caption=Sample test metadata, label=lst:metadata]
{
  "test_name": "PremiumExperience",
  "device": "iPhone 15 Pro",
  "os": "iOS17.5",
  "appearance": "light",
  "user_type": "premium",
  "feature_flags": [
    "COLOR_CHANGE_PREMIUM_BADGE", "CONTENT_CHANGE_PREMIUM_FEATURES"
  ],
  "categories": [
    "CONTENT_CHANGE",
    "COLOR_CHANGE"
  ],
  "timestamp": "2025-05-05T15:13:45Z"
}
\end{lstlisting}

==> motivation.tex <==
\section{Motivation}

Snapshot testing is widely used in UI testing to catch visual changes. It helps developers notice when something in the UI has changed. However, these tests often fail for reasons that are not important, such as small layout or color changes. This creates a large maintenance burden, especially when developers must review and update snapshots manually. 

These frequent failures do not always mean something is broken. But because snapshot tests only show that “something changed” without context, developers cannot easily decide if the change is expected or a real problem. \sa{An example here.} As a result, many teams either ignore test failures or accept changes without checking them carefully. This reduces trust in snapshot testing and wastes developer time.

\sa{It's a combination of text and image, that's why we need Multi-modal models}

We believe that this situation can be improved. Large Language Models (LLMs) with vision capabilities can understand and explain UI changes. They can help identify the reason for a test failure and describe what has changed. This allows developers to focus on meaningful problems and ignore harmless changes. Our work explores how LLMs can make snapshot testing more useful, more reliable, and easier to manage.


==> snapshotter_lst.tex <==
\begin{lstlisting}[caption={Helper to run the test twice: Once with flag disabled, once with flag enabled},label=lst:runTestWithFlagVariants]
 // Helper to run the test twice - once with flag disabled, once with flag enabled
 func runTestWithFlagVariants(flagName: String, testName: String, setupAction: () -> Void, snapshotAction: () -> Void) {
     // First run: flag disabled (default state)
     app = XCUIApplication()
     app.launchArguments = ["UI-TESTING", "DISABLE-ANIMATIONS"]
     app.launch()
     
     setupAction()
     snapshotAction()
     self.assertSnapshotWithName(named: "\(testName)_Default")
     
     // Second run: flag enabled
     app.terminate()
     app = XCUIApplication()
     
     let isAnimationTest = flagName.contains("ANIMATION")
     
     if isAnimationTest {
         app.launchArguments = ["UI-TESTING", "ENABLE_FLAG_\(flagName)"]
     } else {
         app.launchArguments = ["UI-TESTING", "DISABLE-ANIMATIONS", "ENABLE_FLAG_\(flagName)"]
     }
     
     app.launch()
     
     setupAction()
     snapshotAction()
     self.assertSnapshotWithName(named: "\(testName)_FlagEnabled")
 }
\end{lstlisting}

==> test-example.tex <==
{\footnotesize
\begin{algorithm}[t]
\caption{UI Snapshot Test with Feature Flag}
\label{alg:ui-snapshot-test-example}
\KwIn{Feature flag \texttt{F}, Test name \texttt{T}}
\KwOut{Snapshot of UI state under feature flag \texttt{F}}

\SetKwFunction{Launch}{LaunchAppWithFlag}
\SetKwFunction{Find}{elementWith}
\SetKwFunction{Tap}{forceTapElement}
\SetKwFunction{Wait}{waitForExistence}

\Launch{F}\;

\BlankLine
\textbf{Setup phase:} Navigate UI\;
\Indp
  app.scrollDown()\;
  
  btn $\leftarrow$ \Find{"ChangeUserTypeButton"}\;
  \Tap{btn}\;
  
  tab $\leftarrow$ \Find{"profileTab"}\;
  \Tap{tab}\;
  
  app.scrollDown()\;
\Indm

\BlankLine
\textbf{Snapshot phase:} Wait and capture\;
\Indp
  badge $\leftarrow$ \Find{"PremiumBadge"}\;
  \Wait{badge, timeout = 5}\;
  captureSnapshot()\;
\Indm
\end{algorithm}
}


==> test_example.tex <==
\begin{lstlisting}[language=Swift, caption=UI test example with snapshot capture, label=lst:test-ex]
func testColorChangePremiumBadge() {
    runTestWithFlagVariants(
        flagName: "COLOR_CHANGE_PREMIUM_BADGE",
        testName: "PremiumBadge",
        setupAction: {
            app.scrollDown()
            app.elementWith(identifier: "ChangeUserTypeButton").forceTapElement()
            app.elementWith(identifier: "profileTab").forceTapElement()
            app.scrollDown()
        },
        snapshotAction: {
            app.elementWith(identifier: "PremiumBadge").waitForExistence(timeout: 5)
        }
    )
}
\end{lstlisting}

==> tmp.tex <==




You're absolutely right. In this motivation paragraph, we do NOT motivate from A/B testing specifically. A/B testing is only mentioned as ONE example of the types of UI changes that cause snapshot test failures.
The core motivation is about snapshot testing maintenance burden - the fact that developers waste time manually inspecting every snapshot failure. A/B testing is just cited as one scenario among many where legitimate UI changes occur:

"intentional feature updates"
"A/B testing variations"
"unintended regressions"

So A/B testing is used as a brief example to illustrate the broader problem (legitimate changes that shouldn't be treated as bugs), not as the main motivation for the research.
The real motivation is: "snapshot tests fail too often, developers waste time investigating, we need smarter analysis." A/B testing is just one case where this problem occurs, alongside any other intentional UI modification.



